Understanding Help-Seeking and Help-Giving on Social Media for Image-Based Sexual Abuse

Image-based sexual abuse (IBSA), like other forms of technology-facilitated abuse, is a growing threat to people's digital safety. Attacks include unwanted solicitations for sexually explicit images, extorting people under threat of leaking their images, or purposefully leaking images to enact revenge or exert control. In this paper, we explore how people seek and receive help for IBSA on social media. Specifically, we identify over 100,000 Reddit posts that engage relationship and advice communities for help related to IBSA. We draw on a stratified sample of 261 posts to qualitatively examine how various types of IBSA unfold, including the mapping of gender, relationship dynamics, and technology involvement to different types of IBSA. We also explore the support needs of victim-survivors experiencing IBSA and how communities help victim-survivors navigate their abuse through technical, emotional, and relationship advice. Finally, we highlight sociotechnical gaps in connecting victim-survivors with important care, regardless of whom they turn to for help.

==> tables/qual-self-help.tex <==
\begin{table}[t]
\small
\caption{The person or people that the poster was seeking help for by posting on Reddit. Counts were not mutually exclusive (some posters were seeking support for themselves and others).}
\label{tab:self-help}
\begin{tabular}{l|rrrrrrr}
\toprule
    \textbf{Help Recipient}
    &\rotatebox{90}{\textbf{NCEI}} & \rotatebox{90}{\textbf{FS}} & \rotatebox{90}{\textbf{RSA}} & \rotatebox{90}{\textbf{CF}} & \rotatebox{90}{\textbf{PS}} & \rotatebox{90}{\textbf{NFS}} & \rotatebox{90}{\textbf{NCSEI}} \\ 
\midrule
Self       & \cellcolor{gray!50} 40 
                & \cellcolor{gray!50} 48
                & \cellcolor{gray!40} 33 
                & \cellcolor{gray!40} 37
                & \cellcolor{gray!50} 42
                & \cellcolor{gray!50} 44 
                & \cellcolor{gray!50} 46    \\
Other(s)      & 7
                & 2
                & 9 
                & 5 
                & 3 
                & 4  
                & 6 \\
Unspecified     & 0   
                & 0   
                & 0  
                & 0 
                & 1 
                & 0  
                & 0 \\ 
\bottomrule
\end{tabular}
\end{table}
